MassiveGNN: Efficient Training via Prefetching for Massively Connected Distributed Graphs

Graph Neural Networks (GNN) are indispensable in learning from graph-structured data, yet their rising computational costs, especially on massively connected graphs, pose significant challenges in terms of execution performance. To tackle this, distributed-memory solutions such as partitioning the graph to concurrently train multiple replicas of GNNs are in practice. However, approaches requiring a partitioned graph usually suffer from communication overhead and load imbalance, even under optimal partitioning and communication strategies due to irregularities in the neighborhood minibatch sampling. This paper proposes practical trade-offs for improving the sampling and communication overheads for representation learning on distributed graphs (using popular GraphSAGE architecture) by developing a parameterized continuous prefetch and eviction scheme on top of the state-of-the-art Amazon DistDGL distributed GNN framework, demonstrating about 15-40% improvement in end-to-end training performance on the National Energy Research Scientific Computing Center's (NERSC) Perlmutter supercomputer for various OGB datasets.

==> baseline.tex <==
\section{Baseline}\label{sec:baseline}
The proposed prefetch method is designed to support both CPU and GPU training. In this section, we examine the trade-offs associated with each version. We evaluate two main configurations: \emph{prefetch without eviction} and \emph{prefetch with eviction}. \emph{Prefetch without eviction} represents the version where remote nodes of the partitions are prefetched by each trainer only once during buffer initialization and retained without eviction throughout the training. We test against various buffer sizes ($f_{p}^{h}$). On the other hand, \emph{prefetch with eviction} represents repetitive eviction of nodes from the buffer. We evaluate this version with various combinations of $ \Delta$ and $\gamma$. Fig. \ref{fig:baseline} shows the best improvements on GPU and CPU (with different optimal $f_{p}^{h},\Delta, \gamma$) on all 4 datasets. Table \ref{tab:num_halo} shows the average number of remote nodes owned by the trainers in each configuration. 
\begin{table}[ht]
\caption{Number of remote nodes on average per trainer in each configuration across datasets.}
\centering
\begin{tabular}{|c|r|r|r|r|}
\hline
\textbf{\#Trainer}       & \textbf{arxiv} & \textbf{reddit} & \textbf{products}   & \textbf{papers} \\ 
\hline
8 & 34.6K& 91.5K & 471K & 14.9M \\
\hline
16 & 30.6K& 119.7K& 352.3K & 14.8M \\
\hline
32 & 26.2K& 123.9K & 307.8K& 14.1M\\
\hline
64 & - & 120.7K & 220.5K& 10.4M\\
\hline
128 & - & - & - & 7.7M \\
\hline
256 & - & - & - & 4.8M\\
\hline
\end{tabular} 
\label{tab:num_halo}
\end{table}
\subsection{GPU Version}
\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
  \item \emph{Prefetch without Eviction}. In Fig. \ref{fig:baseline} [a-d], the optimal $f_{p}^{h}$ (indicated by the orange bar in each group) consistently demonstrates improvements through our degree-based prefetching strategy across various datasets and node configurations. We observe improvements up to 90\% in arxiv, 26\% in products, 34\% in reddit, and 22\% in papers. We also observe a negative scenario in papers using 256 trainers (64 nodes). \plantodo{Why?} 
 \item \emph{Prefetch with Eviction}. We explore our eviction strategy by optimizing $\Delta$ over optimal $f_{p}^{h}$ and assessing the impact of various $\gamma$ values on both time and hit rate. Fig. \ref{fig:baseline} [a-d] shows that the eviction strategy enhances the hit rate and reduces training time across all tested configurations. In all the experiments, papers use memory-efficient eviction and hence have a slightly higher computational overhead than other inputs.
\end{enumerate}
\subsection{CPU Version} 
\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
 \item \emph{Prefetch without Eviction}.  When training occurs exclusively on CPUs, as depicted in Fig. \ref{fig:baseline} [e-h], we see significant performance improvements over DistDGL. The slower nature of CPU training allows for a \emph{perfect} overlap between the training of current minibatches and the preparation of subsequent ones, leading to enhanced performance gains compared to the GPU version. All configurations tested underscore the advantages of degree-based prefetching, consistently demonstrating improvements across the spectrum. 

\item \emph{Prefetch with Eviction}. As illustrated in Fig. \ref{fig:baseline} [e-h], our eviction strategy reduces training time and improves buffer utilization. Empirical evidence suggests that despite the overhead associated with managing the eviction process, the overall training duration decreases, and resource utilization becomes more efficient.
\end{enumerate}
\subsection{Scalability}
Fig. \ref{fig:baseline} also demonstrates that our approach not only reduces training time but also exhibits consistent scalability across all evaluated datasets and configurations. Notably, in our experiments, DistDGL exhibited limited scalability on the arxiv dataset. We hypothesize that this is due to a disproportionately high communication overhead relative to the computational workload, which is more pronounced in smaller datasets like arxiv. DistDGL's scalability issue has also been discussed in \plantodo{cite the paper where dgl didn't scale.} In reddit and papers, we also find improvements starting to drop past a certain number of trainers (or, nodes). As the number of partitions increases, each trainer will inevitably train on a smaller number of training nodes, resulting in $t_{DDP}<<t_{Prepare}$. With the prefetch overhead remaining constant, the improvement plateaus. The saturation point depends on the scale and connectivity of the input graph.

==> setup.tex <==
\section{Experimental Setup}\label{sec:setup}
The experiments are performed on NERSC Perlmutter, which is based on Cray Shasta platform and consists of 1,792 GPU compute nodes. Each node uses AMD EPYC 7763 and NVIDIA A100 accelerators with HPE Slingshot 11 interconnect. Given that the Perlmutter CPU architecture is a two-socket NUMA system, we have optimized the CPU version of our distributed GNN by setting the CPU affinity for each trainer. Specifically, we utilize 32 cores per trainer, dividing them such that 16 cores are dedicated to NUMBA parallel operations and the remaining 16 are allocated for PyTorch. This configuration ensures that the threads for both NUMBA and PyTorch are bound locally to their respective cores, thereby preventing thread migration across sockets. This turned out to be crucial for avoiding performance degradation due to the increased latency of accessing memory across different NUMA nodes.
\subsection{Dataset and Model}
We conducted our experiments using four datasets: reddit \cite{9407264}, obgn-arxiv, ogbn-products, and obgn-papers100M \cite{hu2020open}. We focus on the node property prediction task and primarily use a 2-layer GraphSage \cite{hamilton2017inductive} with a fanout of \{10, 25\} and a batch size of 2000. We test our prefetching scheme at various scales of 2, 4, 8, 16, 32, and 64 nodes. In all our experiments, each node has four trainer processes. The NeighborSampler algorithm was chosen as our primary sampling strategy for training the GNN model. We used DistDGL with 1 server per node and set the number of sampler processes to 0. Number of nodes used is equal to the number of partition of each graph. We test various values of $f_{p}^{h}$ (0.15, 0.25, 0.35, and 0.50), $\Delta$ (16, 32, 64, 128, 512, and 1024), and $gamma$ (0.95, 0.995, 0.9995) and discuss the results in  \ref{sec:baseline}. The choice of $\gamma$ was found empirically and is later discussed in Section \ref{subsec:gamma}.
\begin{table}[ht]
\caption{Datasets used in the experiments to evaluate our approach against DistDGL.}
\centering
\begin{tabular}{|l|r|r|r|}
\hline
\textbf{Dataset}       & \textbf{$\mathbf{|V|}$} & \textbf{$\mathbf{|E|}$}     & \textbf{Feature Dimension} \\ \hline
arxiv               & 0.16M       & 1.16M	     & 128\\ \hline
products       & 2.4M        & 61.85M        & 100\\ \hline
reddit              & 0.23M          & 114.61M        & 602\\ \hline
papers              & 111M        & 1.6B         & 128\\ \hline

\end{tabular} 
\label{tab:datasets}
\end{table}


% \begin{enumerate}
%     % \item \plantodo{Analyze hyperparameters: Specifically batch size and fan-out.} \comm{TPDS?}
%     % \item \plantodo{Test the system scalability by varying the number of clients per node: Considering scenarios with 1 and 2 clients.} \comm{TPDS?}
%     \item \plantodo{Like, one common criticism could be - how can you select the parameters for sustainable improvement across various nodes/processes (are there negative scenarios?).
%     another criticism: does self-stabilization/ correction actually work - what are the limitations?
%     We must also defend ourselves at the outset about "distributed-memory needs for GNNs", when memory/node is on the rise - we should not just say "data (graphs and features) are getting larger, so distributed-memory is practical" - we should strive to provide a more appealing reason to consider distributed-memory and why communication cannot be fully replaced (as in full prefetch is out of question).}
% \end{enumerate}



